Mimicking or Reasoning: Rethinking Multi-Modal In-Context Learning in Vision-Language Models

Vision-language models (VLMs) are widely assumed to exhibit in-context learning (ICL), a property similar to that of their language-only counterparts. While recent work suggests VLMs can perform multimodal ICL (MM-ICL), studies show they often rely on shallow heuristics -- such as copying or majority voting -- rather than true task understanding. We revisit this assumption by evaluating VLMs under distribution shifts, where support examples come from a dataset different from the query. Surprisingly, performance often degrades with more demonstrations, and models tend to copy answers rather than learn from them. To investigate further, we propose a new MM-ICL with Reasoning pipeline that augments each demonstration with a generated rationale alongside the answer. We conduct extensive and comprehensive experiments on both perception- and reasoning-required datasets with open-source VLMs ranging from 3B to 72B and proprietary models such as Gemini 2.0. We conduct controlled studies varying shot count, retrieval method, rationale quality, and distribution. Our results show limited performance sensitivity across these factors, suggesting that current VLMs do not effectively utilize demonstration-level information as intended in MM-ICL.

==> tabs/all_results.tex <==
\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on A-OKVQA (random)}
\label{tab:Qwen2.5-VL-3B-Instruct_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 85.41 & 82.01 & 80.26 & 80.96 & 78.17 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} & 85.07 & 81.31 & 81.31 & 80.44 & 79.39 \\
\textbf{VLM-R1 unstructered gt\_rationale} & 85.07 & 82.10 & 81.22 & 81.22 & 79.91 \\
\textbf{VLM-R1} &  & 82.45 & 81.83 & 81.48 & 81.14 \\
\textbf{VLM-R1 correct} &  & 83.58 & 82.71 & 81.40 & 80.87 \\
\textbf{VLM-R1 gt\_rationale} &  & 82.01 & 82.18 & 82.10 & 81.14 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 83.76 & 83.06 & 82.27 & 81.57 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on A-OKVQA (jices)}
\label{tab:Qwen2.5-VL-3B-Instruct_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} &  & 82.53 & 80.26 & 80.09 & 79.21 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 80.61 & 79.65 & 79.21 & 79.13 \\
\textbf{VLM-R1 correct} &  & 80.35 & 80.17 & 79.48 & 78.08 \\
\textbf{VLM-R1 gt\_rationale} &  & 81.14 & 80.70 & 80.79 & 80.52 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 80.96 & 80.61 & 80.52 & 80.35 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on ScienceQA (random)}
\label{tab:Qwen2.5-VL-3B-Instruct_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 81.61 & 81.11 & 80.61 & 80.61 & 81.06 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} & 82.30 & 81.71 & 81.95 & 81.31 & 80.61 \\
\textbf{VLM-R1 unstructered gt\_rationale} & 82.30 & 82.35 & 81.51 & 82.15 & 81.21 \\
\textbf{VLM-R1} &  & 82.30 & 83.39 & 82.45 & 82.94 \\
\textbf{VLM-R1 correct} &  & 82.15 & 81.95 & 82.30 & 82.45 \\
\textbf{VLM-R1 gt\_rationale} &  & 82.90 & 83.04 & 82.35 & 82.65 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 82.25 & 83.09 & 83.04 & 82.05 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on ScienceQA (jices)}
\label{tab:Qwen2.5-VL-3B-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} &  & 84.78 & 84.58 & 84.43 & 84.43 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 82.10 & 82.05 & 82.00 & 82.10 \\
\textbf{VLM-R1 correct} &  & 82.90 & 84.18 & 84.43 & 83.59 \\
\textbf{VLM-R1 gt\_rationale} &  & 82.20 & 83.74 & 84.53 & 82.70 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 82.00 & 83.54 & 84.23 & 82.50 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on M3CoT (random)}
\label{tab:Qwen2.5-VL-3B-Instruct_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 51.77 & 51.34 & 51.34 & 50.78 & 50.86 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} & 53.11 & 51.64 & 53.36 & 51.51 & 50.60 \\
\textbf{VLM-R1 unstructered gt\_rationale} & 53.15 & 52.72 & 52.76 & 53.45 & 52.46 \\
\textbf{VLM-R1} &  & 53.19 & 53.80 & 54.36 & 52.89 \\
\textbf{VLM-R1 correct} &  & 51.68 & 53.84 & 52.89 & 53.19 \\
\textbf{VLM-R1 gt\_rationale} &  & 53.62 & 53.80 & 54.92 & 54.18 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 53.62 & 54.57 & 53.41 & 54.83 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on M3CoT (jices)}
\label{tab:Qwen2.5-VL-3B-Instruct_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 51.86 & 52.37 & 53.75 & 55.52 & 56.13 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 55.57 & 54.40 & 55.65 & 56.51 \\
\textbf{VLM-R1 correct} &  & 53.06 & 53.71 & 55.35 & 54.23 \\
\textbf{VLM-R1 gt\_rationale} &  & 53.84 & 54.36 & 55.00 & 54.27 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 53.62 & 53.88 & 55.00 & 54.53 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on TextVQA (random)}
\label{tab:Qwen2.5-VL-3B-Instruct_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 79.13 & 78.70 & 78.58 & 78.09 & 77.80 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} &  & 73.79 &  &  &  \\
\textbf{VLM-R1 unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} & 74.87 & 74.29 & 74.33 & 74.54 & 73.42 \\
\textbf{VLM-R1 correct} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on TextVQA (jices)}
\label{tab:Qwen2.5-VL-3B-Instruct_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 79.22 & 76.49 & 76.44 & 76.56 & 76.42 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} & 74.87 & 71.00 &  &  &  \\
\textbf{VLM-R1 unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 71.23 & 71.49 & 71.19 & 70.88 \\
\textbf{VLM-R1 correct} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on OK-VQA (random)}
\label{tab:Qwen2.5-VL-3B-Instruct_OK-VQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 54.09 & 56.63 & 56.54 & 55.70 & 55.67 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} & 40.00 & 41.85 & 43.03 & 46.63 & 51.55 \\
\textbf{VLM-R1 unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} & 40.00 & 41.59 & 42.97 & 42.95 & 42.45 \\
\textbf{VLM-R1 correct} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on OK-VQA (jices)}
\label{tab:Qwen2.5-VL-3B-Instruct_OK-VQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 54.09 & 56.37 & 57.78 & 57.87 & 58.27 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered} &  &  &  &  &  \\
\textbf{VLM-R1 unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  &  &  &  &  \\
\textbf{VLM-R1 correct} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on A-OKVQA (random)}
\label{tab:Qwen2.5-VL-7B-Instruct_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 88.56 & 88.65 & 87.86 & 87.77 & 88.03 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} & 85.68 & 85.76 & 85.24 & 84.28 & 83.76 \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} & 85.68 & 85.33 & 85.24 & 85.76 & 84.45 \\
\textbf{VL-Rethinker-7B} &  & 85.50 & 84.98 & 84.98 & 85.68 \\
\textbf{VL-Rethinker-7B correct} &  & 85.15 & 85.15 & 85.41 & 85.07 \\
\textbf{VL-Rethinker-7B gt\_rationale} &  & 85.85 & 85.41 & 85.15 & 86.03 \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  & 85.15 & 86.03 & 85.94 & 85.59 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on A-OKVQA (jices)}
\label{tab:Qwen2.5-VL-7B-Instruct_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 88.56 & 88.30 & 88.21 & 87.95 & 87.95 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} & 85.68 & 85.85 & 85.68 & 84.54 & 84.54 \\
\textbf{VL-Rethinker-7B correct} & 85.68 & 85.59 & 86.11 & 85.15 & 85.24 \\
\textbf{VL-Rethinker-7B gt\_rationale} & 85.68 & 85.15 & 85.41 & 85.50 & 85.50 \\
\textbf{VL-Rethinker-7B gt\_rationale correct} & 85.68 & 85.33 & 85.76 & 85.59 & 85.68 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on ScienceQA (random)}
\label{tab:Qwen2.5-VL-7B-Instruct_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 88.99 & 86.71 & 87.65 & 86.56 & 86.86 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} & 89.64 & 89.04 & 88.94 & 88.89 & 89.14 \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} & 89.64 & 89.04 & 89.34 & 89.49 & 89.34 \\
\textbf{VL-Rethinker-7B} &  & 90.23 & 90.23 & 90.18 & 90.23 \\
\textbf{VL-Rethinker-7B correct} &  & 89.74 & 90.18 & 90.18 & 89.74 \\
\textbf{VL-Rethinker-7B gt\_rationale} &  & 90.13 & 89.79 & 90.48 & 90.38 \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  & 89.74 & 89.74 & 90.38 & 90.58 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on ScienceQA (jices)}
\label{tab:Qwen2.5-VL-7B-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 88.99 & 89.09 & 89.69 & 89.69 & 90.28 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} & 89.64 & 88.35 & 89.19 & 88.55 & 88.00 \\
\textbf{VL-Rethinker-7B correct} & 89.64 & 89.59 & 89.84 &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} & 89.64 & 90.13 & 91.08 & 90.83 & 90.68 \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on M3CoT (random)}
\label{tab:Qwen2.5-VL-7B-Instruct_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 63.03 & 60.40 & 60.05 & 60.22 & 60.53 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} & 67.90 & 66.22 & 67.60 & 66.39 & 66.82 \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} & 67.90 & 67.86 & 67.86 & 67.64 & 67.43 \\
\textbf{VL-Rethinker-7B} &  & 68.08 & 69.15 & 68.59 & 68.55 \\
\textbf{VL-Rethinker-7B correct} &  & 67.90 & 68.98 & 69.11 & 67.90 \\
\textbf{VL-Rethinker-7B gt\_rationale} &  & 67.13 & 67.73 & 68.33 & 68.55 \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  & 68.12 & 68.33 & 69.97 & 67.56 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on M3CoT (jices)}
\label{tab:Qwen2.5-VL-7B-Instruct_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} &  &  &  &  &  \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B correct} & 67.90 & 67.82 & 67.43 & 66.87 & 67.13 \\
\textbf{VL-Rethinker-7B gt\_rationale} & 67.90 & 67.17 &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} & 67.90 & 66.13 & 67.39 & 66.57 & 66.78 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on TextVQA (random)}
\label{tab:Qwen2.5-VL-7B-Instruct_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 85.39 & 84.79 & 84.45 & 84.09 & 84.12 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} & 76.46 & 73.01 & 72.38 & 72.04 & 72.32 \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on TextVQA (jices)}
\label{tab:Qwen2.5-VL-7B-Instruct_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 85.39 & 83.09 & 83.15 & 83.48 & 83.56 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on OK-VQA (random)}
\label{tab:Qwen2.5-VL-7B-Instruct_OK-VQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 58.74 & 62.33 & 62.68 & 62.49 & 62.33 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} & 32.43 & 32.65 & 32.30 & 31.68 & 32.21 \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} & 32.43 & 30.14 & 29.37 & 29.04 & 28.86 \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on OK-VQA (jices)}
\label{tab:Qwen2.5-VL-7B-Instruct_OK-VQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 58.74 & 62.08 & 63.10 & 63.36 & 64.11 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on A-OKVQA (random)}
\label{tab:Llama-3.2-11B-Vision-Instruct_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} & 84.02 & 84.02 & 83.49 & 83.58 & 82.71 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} & 87.42 & 85.85 & 85.33 & 84.28 & 83.14 \\
\textbf{LLaVA-CoT unstructered gt\_rationale} & 87.42 & 85.24 & 84.80 & 84.19 & 83.84 \\
\textbf{LLaVA-CoT} &  & 86.20 & 85.59 & 84.54 & 83.23 \\
\textbf{LLaVA-CoT correct} &  & 84.89 & 84.89 & 84.63 & 84.10 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 85.41 & 84.72 & 84.98 & 83.41 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 84.89 & 84.72 & 86.03 & 84.45 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on A-OKVQA (jices)}
\label{tab:Llama-3.2-11B-Vision-Instruct_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} &  & 78.34 & 78.17 & 79.56 & 80.52 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 83.41 & 83.41 & 82.27 & 82.88 \\
\textbf{LLaVA-CoT correct} &  & 82.53 & 83.58 & 84.28 & 82.62 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 84.37 & 83.67 & 82.97 & 82.18 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 84.28 & 83.76 & 83.58 & 82.62 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on ScienceQA (random)}
\label{tab:Llama-3.2-11B-Vision-Instruct_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} & 83.99 & 82.85 & 84.43 & 84.13 & 83.64 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} & 94.55 & 91.52 & 90.98 & 87.65 & 84.78 \\
\textbf{LLaVA-CoT unstructered gt\_rationale} & 94.55 & 92.36 & 91.97 & 88.99 & 87.56 \\
\textbf{LLaVA-CoT} &  & 92.81 & 91.97 & 91.57 & 90.48 \\
\textbf{LLaVA-CoT correct} &  & 92.17 & 92.02 & 92.27 & 90.58 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 93.51 & 92.12 & 91.62 & 91.32 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 93.31 & 91.62 & 91.32 & 91.03 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on ScienceQA (jices)}
\label{tab:Llama-3.2-11B-Vision-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} &  & 83.89 & 85.03 & 86.27 & 87.21 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} &  & 89.49 & 89.04 & 87.51 & 88.25 \\
\textbf{LLaVA-CoT unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 89.09 & 90.48 & 88.89 & 87.61 \\
\textbf{LLaVA-CoT correct} &  & 89.34 & 90.88 & 89.89 & 87.80 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 91.08 & 89.64 & 90.63 & 88.80 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 90.13 & 90.43 & 89.44 & 89.54 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on M3CoT (random)}
\label{tab:Llama-3.2-11B-Vision-Instruct_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} & 42.45 & 42.75 & 43.74 & 42.58 & 42.49 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} & 56.26 & 55.26 & 51.42 & 44.26 & 42.28 \\
\textbf{LLaVA-CoT unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 54.62 & 53.62 & 52.29 & 50.99 \\
\textbf{LLaVA-CoT correct} &  & 54.18 & 54.01 & 52.76 & 51.81 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 53.88 & 52.85 & 52.24 & 50.78 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 55.69 & 54.83 & 53.67 & 52.50 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on M3CoT (jices)}
\label{tab:Llama-3.2-11B-Vision-Instruct_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} & 42.41 & 44.91 & 46.12 & 48.62 & 47.37 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 53.19 & 52.72 & 52.50 & 50.91 \\
\textbf{LLaVA-CoT correct} &  & 55.65 & 54.01 & 53.88 & 50.82 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 52.07 & 53.54 & 54.27 & 52.63 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 51.68 & 53.75 & 52.59 & 52.37 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on TextVQA (random)}
\label{tab:Llama-3.2-11B-Vision-Instruct_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} & 53.87 & 74.52 & 74.63 & 74.43 & 73.83 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} &  & 0.00 &  &  &  \\
\textbf{LLaVA-CoT unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} & 72.85 & 74.39 & 74.04 & 74.39 & 72.96 \\
\textbf{LLaVA-CoT correct} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on TextVQA (jices)}
\label{tab:Llama-3.2-11B-Vision-Instruct_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} &  & 63.09 & 66.66 & 65.69 & 63.66 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} & 0.00 & 0.00 &  &  &  \\
\textbf{LLaVA-CoT unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 69.16 & 68.93 & 68.31 &  \\
\textbf{LLaVA-CoT correct} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on OK-VQA (random)}
\label{tab:Llama-3.2-11B-Vision-Instruct_OK-VQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} & 20.05 & 37.49 & 40.05 & 42.89 & 44.03 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} & 48.91 & 47.33 & 48.07 & 48.18 & 49.43 \\
\textbf{LLaVA-CoT unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} & 48.91 & 47.46 & 46.95 &  &  \\
\textbf{LLaVA-CoT correct} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on OK-VQA (jices)}
\label{tab:Llama-3.2-11B-Vision-Instruct_OK-VQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} & 20.05 & 42.67 & 44.61 & 45.82 & 46.08 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered} &  &  &  &  &  \\
\textbf{LLaVA-CoT unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} & 48.91 & 42.12 & 43.59 &  &  \\
\textbf{LLaVA-CoT correct} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on A-OKVQA (random)}
\label{tab:InternVL2_5-4B_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 85.85 & 84.37 & 84.02 & 83.76 & 83.49 \\
\textbf{InternVL2\_5-4B gt\_rationale} & 85.85 & 84.45 & 84.19 & 82.53 & 83.14 \\
\textbf{InternVL2\_5-4B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} & 84.89 & 83.58 & 81.40 & 82.36 & 82.53 \\
\textbf{InternVL2\_5-4B-MPO correct} &  & 83.67 & 84.37 & 83.76 & 83.67 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} & 84.89 & 83.32 & 80.70 & 80.17 & 80.44 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  & 83.49 & 79.39 & 80.09 & 78.86 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on A-OKVQA (jices)}
\label{tab:InternVL2_5-4B_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} &  & 84.02 & 83.41 & 83.23 & 83.06 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  & 84.72 & 83.76 & 83.58 & 82.97 \\
\textbf{InternVL2\_5-4B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on ScienceQA (random)}
\label{tab:InternVL2_5-4B_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 97.17 & 96.28 & 96.43 & 95.93 & 95.54 \\
\textbf{InternVL2\_5-4B gt\_rationale} & 97.17 & 96.53 & 96.68 & 96.53 & 95.49 \\
\textbf{InternVL2\_5-4B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} & 97.32 & 96.78 & 96.48 & 96.88 & 95.93 \\
\textbf{InternVL2\_5-4B-MPO correct} &  & 96.63 & 96.78 & 96.43 & 96.23 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} & 97.32 & 96.43 & 96.88 & 96.33 & 95.98 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  & 96.63 & 96.38 & 96.58 & 95.88 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on ScienceQA (jices)}
\label{tab:InternVL2_5-4B_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} &  & 95.69 & 95.29 & 94.60 & 94.20 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  & 96.28 & 96.58 & 96.38 & 95.88 \\
\textbf{InternVL2\_5-4B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on M3CoT (random)}
\label{tab:InternVL2_5-4B_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 55.74 & 54.27 & 53.80 & 53.97 & 54.44 \\
\textbf{InternVL2\_5-4B gt\_rationale} & 55.74 & 54.62 & 54.62 & 54.31 & 54.83 \\
\textbf{InternVL2\_5-4B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} & 64.50 & 58.54 & 55.65 & 55.22 & 57.08 \\
\textbf{InternVL2\_5-4B-MPO correct} &  & 61.56 & 62.90 & 61.82 & 62.21 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} & 64.50 & 61.39 & 59.49 & 56.73 & 55.31 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  & 61.13 & 59.32 & 57.25 & 55.48 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on M3CoT (jices)}
\label{tab:InternVL2_5-4B_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} &  & 58.24 & 57.33 & 57.85 & 59.49 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  & 55.87 & 56.04 & 55.48 & 53.97 \\
\textbf{InternVL2\_5-4B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on TextVQA (random)}
\label{tab:InternVL2_5-4B_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 78.68 & 78.88 & 78.53 & 77.77 & 77.39 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} & 72.85 & 72.90 & 72.78 & 71.64 & 71.51 \\
\textbf{InternVL2\_5-4B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on TextVQA (jices)}
\label{tab:InternVL2_5-4B_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} &  & 77.96 & 76.75 & 76.04 & 75.14 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on OK-VQA (random)}
\label{tab:InternVL2_5-4B_OK-VQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 49.88 & 54.68 & 54.79 & 54.41 & 53.63 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered} & 0.00 & 2.39 & 21.81 & 41.07 & 48.91 \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} & 42.12 & 41.85 & 42.55 & 41.54 & 42.05 \\
\textbf{InternVL2\_5-4B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on OK-VQA (jices)}
\label{tab:InternVL2_5-4B_OK-VQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 49.88 & 55.15 & 56.00 & 55.46 & 55.62 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on A-OKVQA (random)}
\label{tab:InternVL2_5-8B_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 87.42 & 86.90 & 84.98 & 85.76 & 85.76 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 87.42 & 86.90 & 86.03 & 85.94 & 84.72 \\
\textbf{InternVL2\_5-8B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} & 87.25 & 86.03 & 84.89 & 84.54 & 81.92 \\
\textbf{InternVL2\_5-8B-MPO correct} &  & 87.16 & 85.50 & 84.80 & 83.76 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} & 87.25 & 86.81 & 85.94 & 84.63 & 83.84 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  & 86.55 & 85.41 & 85.15 & 84.10 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on A-OKVQA (jices)}
\label{tab:InternVL2_5-8B_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 87.42 & 86.64 & 85.94 & 85.33 & 84.72 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 87.42 & 86.99 & 86.46 & 86.11 & 85.07 \\
\textbf{InternVL2\_5-8B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on ScienceQA (random)}
\label{tab:InternVL2_5-8B_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 98.07 & 97.77 & 97.72 & 97.17 & 96.08 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 98.07 & 97.82 & 97.57 & 97.32 & 96.43 \\
\textbf{InternVL2\_5-8B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} & 98.56 & 98.07 & 98.22 & 97.57 & 96.48 \\
\textbf{InternVL2\_5-8B-MPO correct} &  & 97.97 & 98.12 & 97.47 & 96.38 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} & 98.56 & 98.02 & 98.12 & 97.32 & 96.83 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  & 98.07 & 97.57 & 97.32 & 96.43 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on ScienceQA (jices)}
\label{tab:InternVL2_5-8B_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 98.07 & 96.18 & 95.24 & 95.09 & 95.14 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 98.07 & 97.82 & 97.32 & 97.12 & 96.38 \\
\textbf{InternVL2\_5-8B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on M3CoT (random)}
\label{tab:InternVL2_5-8B_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 62.42 & 59.92 & 59.75 & 58.46 & 57.42 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 62.42 & 59.36 & 58.93 & 58.63 & 58.54 \\
\textbf{InternVL2\_5-8B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} & 73.51 & 68.98 & 67.56 & 65.96 & 63.37 \\
\textbf{InternVL2\_5-8B-MPO correct} &  & 68.94 & 68.25 & 65.75 & 60.96 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} & 73.51 & 69.97 & 67.56 & 67.39 & 63.76 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  & 68.94 & 68.12 & 66.44 & 63.37 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on M3CoT (jices)}
\label{tab:InternVL2_5-8B_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 62.42 & 60.83 & 60.18 & 60.87 & 60.01 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 62.42 & 59.75 & 57.85 & 58.15 & 58.76 \\
\textbf{InternVL2\_5-8B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on TextVQA (random)}
\label{tab:InternVL2_5-8B_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 79.03 & 78.73 & 78.61 & 78.45 & 77.65 \\
\textbf{InternVL2\_5-8B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} & 73.36 & 73.67 & 73.37 & 72.47 & 73.03 \\
\textbf{InternVL2\_5-8B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on TextVQA (jices)}
\label{tab:InternVL2_5-8B_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} &  & 77.60 & 75.61 & 75.51 & 74.30 \\
\textbf{InternVL2\_5-8B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on OK-VQA (random)}
\label{tab:InternVL2_5-8B_OK-VQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 57.20 & 59.62 & 59.13 & 58.30 & 57.51 \\
\textbf{InternVL2\_5-8B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered} & 0.00 & 0.00 & 0.13 &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} & 44.49 & 48.11 & 49.01 & 48.51 & 47.98 \\
\textbf{InternVL2\_5-8B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on OK-VQA (jices)}
\label{tab:InternVL2_5-8B_OK-VQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 57.20 & 60.02 & 59.44 & 58.64 & 57.99 \\
\textbf{InternVL2\_5-8B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO unstructered gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/all_results_general.tex <==
\begin{table}[!h]
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on TextVQA (random)}
\label{tab:Qwen2.5-VL-3B-Instruct_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 79.13 & 78.70 & 78.58 &  &  \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 74.29 & 74.33 &  &  \\
\textbf{VLM-R1 correct} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on TextVQA (jices)}
\label{tab:Qwen2.5-VL-3B-Instruct_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 79.22 & 76.49 & 76.44 & 76.56 &  \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 71.23 & 71.49 &  &  \\
\textbf{VLM-R1 correct} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1 gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on TextVQA (random)}
\label{tab:Qwen2.5-VL-7B-Instruct_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 85.39 & 84.79 & 84.45 & 84.09 & 84.12 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on TextVQA (jices)}
\label{tab:Qwen2.5-VL-7B-Instruct_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 85.39 & 83.09 & 83.15 & 83.48 & 83.56 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on TextVQA (random)}
\label{tab:Llama-3.2-11B-Vision-Instruct_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} &  & 74.52 &  &  &  \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 74.39 & 74.04 &  &  \\
\textbf{LLaVA-CoT correct} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on TextVQA (jices)}
\label{tab:Llama-3.2-11B-Vision-Instruct_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} &  & 63.09 &  &  &  \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  &  &  &  &  \\
\textbf{LLaVA-CoT correct} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on TextVQA (random)}
\label{tab:InternVL2_5-4B_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 78.68 & 78.88 & 78.53 & 77.77 & 77.39 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on TextVQA (jices)}
\label{tab:InternVL2_5-4B_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on TextVQA (random)}
\label{tab:InternVL2_5-8B_TextVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 79.03 & 78.73 & 78.61 & 78.45 &  \\
\textbf{InternVL2\_5-8B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on TextVQA (jices)}
\label{tab:InternVL2_5-8B_TextVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO correct} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/all_results_reason.tex <==
\begin{table}[!h]
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on A-OKVQA (random)}
\label{tab:Qwen2.5-VL-3B-Instruct_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} &  & 82.01 & 80.26 & 80.96 & 78.17 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 82.45 & 81.83 & 81.48 & 81.14 \\
\textbf{VLM-R1 correct} &  & 83.58 & 82.71 & 81.40 & 80.87 \\
\textbf{VLM-R1 gt\_rationale} &  & 82.01 & 82.18 & 82.10 & 81.14 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 83.76 & 83.06 & 82.27 & 81.57 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on A-OKVQA (jices)}
\label{tab:Qwen2.5-VL-3B-Instruct_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} &  & 82.53 & 80.26 & 80.09 & 79.21 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 80.61 & 79.65 & 79.21 & 79.13 \\
\textbf{VLM-R1 correct} &  & 80.35 & 80.17 & 79.48 & 78.08 \\
\textbf{VLM-R1 gt\_rationale} &  & 81.14 & 80.70 & 80.79 & 80.52 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 80.96 & 80.61 & 80.52 & 80.35 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on ScienceQA (random)}
\label{tab:Qwen2.5-VL-3B-Instruct_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} &  & 81.11 & 80.61 & 80.61 & 81.06 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 82.30 & 83.39 & 82.45 & 82.94 \\
\textbf{VLM-R1 correct} &  & 82.15 & 81.95 & 82.30 & 82.45 \\
\textbf{VLM-R1 gt\_rationale} &  & 82.90 & 83.04 & 82.35 & 82.65 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 82.25 & 83.09 & 83.04 & 82.05 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on ScienceQA (jices)}
\label{tab:Qwen2.5-VL-3B-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} &  & 84.78 & 84.58 & 84.43 & 84.43 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 82.10 & 82.05 & 82.00 & 82.10 \\
\textbf{VLM-R1 correct} &  & 82.90 & 84.18 & 84.43 & 83.59 \\
\textbf{VLM-R1 gt\_rationale} &  & 82.20 & 83.74 & 84.53 & 82.70 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 82.00 & 83.54 & 84.23 & 82.50 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on M3CoT (random)}
\label{tab:Qwen2.5-VL-3B-Instruct_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 51.77 & 51.34 & 51.34 & 50.78 & 50.86 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 53.19 & 53.80 & 54.36 & 52.89 \\
\textbf{VLM-R1 correct} &  & 51.68 & 53.84 & 52.89 & 53.19 \\
\textbf{VLM-R1 gt\_rationale} &  & 53.62 & 53.80 & 54.92 & 54.18 \\
\textbf{VLM-R1 gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-3B-Instruct vs. VLM-R1 on M3CoT (jices)}
\label{tab:Qwen2.5-VL-3B-Instruct_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-3B-Instruct} & 51.86 & 52.37 & 53.75 & 55.52 & 56.13 \\
\textbf{Qwen2.5-VL-3B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VLM-R1} &  & 55.57 & 54.40 & 55.65 & 56.51 \\
\textbf{VLM-R1 correct} &  & 53.06 & 53.71 & 55.35 & 54.23 \\
\textbf{VLM-R1 gt\_rationale} &  & 53.84 & 54.36 & 55.00 & 54.27 \\
\textbf{VLM-R1 gt\_rationale correct} &  & 53.62 & 53.88 & 55.00 & 54.53 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on A-OKVQA (random)}
\label{tab:Qwen2.5-VL-7B-Instruct_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 88.56 & 88.65 & 87.86 & 87.77 & 88.03 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  & 85.50 & 84.98 & 84.98 & 85.68 \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  & 85.85 & 85.41 & 85.15 & 86.03 \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on A-OKVQA (jices)}
\label{tab:Qwen2.5-VL-7B-Instruct_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 88.56 & 88.30 & 88.21 & 87.95 & 87.95 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on ScienceQA (random)}
\label{tab:Qwen2.5-VL-7B-Instruct_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 88.99 & 86.71 & 87.65 & 86.56 & 86.86 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  & 90.23 & 90.23 & 90.18 & 90.23 \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  & 90.13 & 89.79 & 90.48 & 90.38 \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on ScienceQA (jices)}
\label{tab:Qwen2.5-VL-7B-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 88.99 & 89.09 & 89.69 & 89.69 & 90.28 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on M3CoT (random)}
\label{tab:Qwen2.5-VL-7B-Instruct_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} & 63.03 & 60.40 & 60.05 & 60.22 & 60.53 \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  & 68.08 & 69.15 & 68.59 & 68.55 \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  & 67.13 & 67.73 & 68.33 & 68.55 \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Qwen2.5-VL-7B-Instruct vs. VL-Rethinker-7B on M3CoT (jices)}
\label{tab:Qwen2.5-VL-7B-Instruct_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-7B-Instruct} &  &  &  &  &  \\
\textbf{Qwen2.5-VL-7B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B correct} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-7B gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!h]
\caption{Qwen2.5-VL-72B-Instruct vs. VL-Rethinker-72B on ScienceQA (jices)}
\label{tab:Qwen2.5-VL-72B-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-72B-Instruct} &91.18  &91.82 &93.95 &94.70 &94.94 \\
% \textbf{Qwen2.5-VL-72B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-72B} &94.40  &  &  &  & \\
% \textbf{VL-Rethinker correct} &  &  &  &  & \\
% \textbf{VL-Rethinker gt\_rationale} &  &  &  &  & \\
% \textbf{VL-Rethinker gt\_rationale correct} &  &  &  &  & \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h]
\caption{Qwen2.5-VL-72B-Instruct vs. VL-Rethinker-72B on ScienceQA (random)}
\label{tab:Qwen2.5-VL-72B-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-72B-Instruct} &91.18  &91.18 &91.47 &91.57 &91.57 \\
% \textbf{Qwen2.5-VL-72B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-72B} &94.40  &93.75  &93.06  &93.16  &93.41 \\
% \textbf{VL-Rethinker correct} &  &  &  &  & \\
% \textbf{VL-Rethinker gt\_rationale} &  &  &  &  & \\
% \textbf{VL-Rethinker gt\_rationale correct} &  &  &  &  & \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h]
\caption{Qwen2.5-VL-72B-Instruct vs. VL-Rethinker-72B on A-OKVQA (jices)}
\label{tab:Qwen2.5-VL-72B-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-72B-Instruct} &91.44  &91.35 &91.35 &91.35
&91.00 \\
% \textbf{Qwen2.5-VL-72B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-72B} &  &  &  &  & \\
% \textbf{VL-Rethinker correct} &  &  &  &  & \\
% \textbf{VL-Rethinker gt\_rationale} &  &  &  &  & \\
% \textbf{VL-Rethinker gt\_rationale correct} &  &  &  &  & \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h]
\caption{Qwen2.5-VL-72B-Instruct vs. VL-Rethinker-72B on A-OKVQA (random)}
\label{tab:Qwen2.5-VL-72B-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Qwen2.5-VL-72B-Instruct} &91.44  &91.18 &90.83 &91.18 &90.39 \\
% \textbf{Qwen2.5-VL-72B-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{VL-Rethinker-72B} &  &  &  &  & \\
% \textbf{VL-Rethinker correct} &  &  &  &  & \\
% \textbf{VL-Rethinker gt\_rationale} &  &  &  &  & \\
% \textbf{VL-Rethinker gt\_rationale correct} &  &  &  &  & \\
\bottomrule
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!h]
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on A-OKVQA (random)}
\label{tab:Llama-3.2-11B-Vision-Instruct_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} &  & 84.02 & 83.49 & 83.58 & 82.71 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 86.20 & 85.59 & 84.54 & 83.23 \\
\textbf{LLaVA-CoT correct} &  & 84.89 & 84.89 & 84.63 & 84.10 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 85.41 & 84.72 & 84.98 & 83.41 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 84.89 & 84.72 & 86.03 & 84.45 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on A-OKVQA (jices)}
\label{tab:Llama-3.2-11B-Vision-Instruct_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} &  & 78.34 & 78.17 & 79.56 & 80.52 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 83.41 & 83.41 & 82.27 & 82.88 \\
\textbf{LLaVA-CoT correct} &  & 82.53 & 83.58 & 84.28 & 82.62 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 84.37 & 83.67 & 82.97 & 82.18 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 84.28 & 83.76 & 83.58 & 82.62 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on ScienceQA (random)}
\label{tab:Llama-3.2-11B-Vision-Instruct_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} &  & 82.85 & 84.43 & 84.13 & 83.64 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 92.81 & 91.97 & 91.57 & 90.48 \\
\textbf{LLaVA-CoT correct} &  & 92.17 & 92.02 & 92.27 & 90.58 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 93.51 & 92.12 & 91.62 & 91.32 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 93.31 & 91.62 & 91.32 & 91.03 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on ScienceQA (jices)}
\label{tab:Llama-3.2-11B-Vision-Instruct_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} &  & 83.89 & 85.03 & 86.27 & 87.21 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 89.09 & 90.48 & 88.89 & 87.61 \\
\textbf{LLaVA-CoT correct} &  & 89.34 & 90.88 & 89.89 & 87.80 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 91.08 & 89.64 & 90.63 & 88.80 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 90.13 & 90.43 & 89.44 & 89.54 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on M3CoT (random)}
\label{tab:Llama-3.2-11B-Vision-Instruct_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} & 42.45 & 42.75 & 43.74 & 42.58 & 42.49 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 54.62 & 53.62 & 52.29 & 50.99 \\
\textbf{LLaVA-CoT correct} &  & 54.18 & 54.01 & 52.76 & 51.81 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 53.88 & 52.85 & 52.24 & 50.78 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 55.69 & 54.83 & 53.67 & 52.50 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{Llama-3.2-11B-Vision-Instruct vs. LLaVA-CoT on M3CoT (jices)}
\label{tab:Llama-3.2-11B-Vision-Instruct_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{Llama-3.2-11B-Vision-Instruct} & 42.41 & 44.91 & 46.12 & 48.62 & 47.37 \\
\textbf{Llama-3.2-11B-Vision-Instruct gt\_rationale} &  &  &  &  &  \\
\textbf{LLaVA-CoT} &  & 53.19 & 52.72 & 52.50 & 50.91 \\
\textbf{LLaVA-CoT correct} &  & 55.65 & 54.01 & 53.88 & 50.82 \\
\textbf{LLaVA-CoT gt\_rationale} &  & 52.07 & 53.54 & 54.27 & 52.63 \\
\textbf{LLaVA-CoT gt\_rationale correct} &  & 51.68 & 53.75 & 52.59 & 52.37 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on A-OKVQA (random)}
\label{tab:InternVL2_5-4B_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 85.85 & 84.37 & 84.02 & 83.76 & 83.49 \\
\textbf{InternVL2\_5-4B gt\_rationale} & 85.85 & 84.45 & 84.19 & 82.53 & 83.14 \\
\textbf{InternVL2\_5-4B-MPO} & 84.89 & 81.57 & 81.14 & 82.53 & 81.75 \\
\textbf{InternVL2\_5-4B-MPO correct} &  & 83.06 & 81.66 & 82.45 & 82.01 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} & 84.89 & 84.45 & 77.99 & 81.05 & 79.56 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  & 84.19 & 78.08 & 80.00 & 79.48 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on A-OKVQA (jices)}
\label{tab:InternVL2_5-4B_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} &  & 84.02 & 83.41 & 83.23 & 83.06 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  & 84.72 & 83.76 & 83.58 & 82.97 \\
\textbf{InternVL2\_5-4B-MPO} &  & 80.52 & 80.79 & 83.23 & 82.97 \\
\textbf{InternVL2\_5-4B-MPO correct} &  & 80.26 & 80.87 & 82.88 & 83.23 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  & 83.84 & 80.44 & 80.35 & 80.96 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  & 83.93 & 80.00 & 81.05 & 81.05 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on ScienceQA (random)}
\label{tab:InternVL2_5-4B_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 97.17 & 96.28 & 96.43 & 95.93 & 95.54 \\
\textbf{InternVL2\_5-4B gt\_rationale} & 97.17 & 96.53 & 96.68 & 96.53 & 95.49 \\
\textbf{InternVL2\_5-4B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO correct} &  & 94.25 & 93.65 & 94.74 & 95.64 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  &  &  &  &  \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  & 95.49 & 95.79 & 95.49 & 95.04 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on ScienceQA (jices)}
\label{tab:InternVL2_5-4B_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} &  & 95.69 & 95.29 & 94.60 & 94.20 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  & 96.28 & 96.58 & 96.38 & 95.88 \\
\textbf{InternVL2\_5-4B-MPO} &  & 90.48 & 89.69 & 92.02 & 91.13 \\
\textbf{InternVL2\_5-4B-MPO correct} &  & 90.28 & 89.49 & 91.87 & 90.98 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  & 92.12 & 92.17 & 91.92 & 90.78 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  & 92.22 & 92.27 & 91.92 & 90.83 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on M3CoT (random)}
\label{tab:InternVL2_5-4B_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} & 55.74 & 54.27 &  &  &  \\
\textbf{InternVL2\_5-4B gt\_rationale} & 55.74 & 54.62 & 54.62 & 54.31 & 54.83 \\
\textbf{InternVL2\_5-4B-MPO} & 64.50 & 57.12 & 55.31 & 55.69 & 58.76 \\
\textbf{InternVL2\_5-4B-MPO correct} &  & 58.54 & 56.34 & 55.57 & 56.73 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} & 64.50 & 61.22 & 57.81 & 55.91 & 55.05 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  & 61.43 & 59.49 & 56.51 & 56.13 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-4B vs. InternVL2\_5-4B-MPO on M3CoT (jices)}
\label{tab:InternVL2_5-4B_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-4B} &  & 58.24 & 57.33 & 57.85 & 59.49 \\
\textbf{InternVL2\_5-4B gt\_rationale} &  & 55.87 & 56.04 & 55.48 & 53.97 \\
\textbf{InternVL2\_5-4B-MPO} &  & 55.26 & 56.86 & 58.76 & 59.49 \\
\textbf{InternVL2\_5-4B-MPO correct} &  & 57.89 & 56.26 & 55.05 & 57.33 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale} &  & 59.32 & 57.64 & 56.26 & 55.87 \\
\textbf{InternVL2\_5-4B-MPO gt\_rationale correct} &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on A-OKVQA (random)}
\label{tab:InternVL2_5-8B_A-OKVQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 87.42 & 86.90 & 84.98 & 85.76 & 85.76 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 87.42 & 86.90 & 86.03 & 85.94 & 84.72 \\
\textbf{InternVL2\_5-8B-MPO} &  & 85.50 & 85.24 & 84.89 & 81.66 \\
\textbf{InternVL2\_5-8B-MPO correct} &  & 86.81 & 85.15 & 83.23 & 81.14 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  & 85.94 & 85.68 & 85.15 & 84.45 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  & 86.55 & 86.20 & 85.41 & 85.24 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on A-OKVQA (jices)}
\label{tab:InternVL2_5-8B_A-OKVQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 87.42 & 86.64 & 85.94 & 85.33 & 84.72 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 87.42 & 86.99 & 86.46 & 86.11 & 85.07 \\
\textbf{InternVL2\_5-8B-MPO} &  & 85.24 & 84.19 & 83.14 & 75.98 \\
\textbf{InternVL2\_5-8B-MPO correct} &  & 86.03 & 84.10 & 83.14 & 75.55 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  & 85.68 & 84.02 & 84.63 & 83.14 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  & 85.50 & 84.28 & 84.98 & 83.14 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on ScienceQA (random)}
\label{tab:InternVL2_5-8B_ScienceQA_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 98.07 & 97.77 & 97.72 & 97.17 & 96.08 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 98.07 & 97.82 & 97.57 & 97.32 & 96.43 \\
\textbf{InternVL2\_5-8B-MPO} &  & 97.72 & 97.32 & 95.09 & 92.61 \\
\textbf{InternVL2\_5-8B-MPO correct} &  & 97.87 & 97.47 & 94.84 & 92.76 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  & 98.02 & 97.82 & 97.52 & 94.65 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  & 98.22 & 98.17 & 96.63 & 93.95 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on ScienceQA (jices)}
\label{tab:InternVL2_5-8B_ScienceQA_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 98.07 & 96.18 & 95.24 & 95.09 & 95.14 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 98.07 & 97.82 & 97.32 & 97.12 & 96.38 \\
\textbf{InternVL2\_5-8B-MPO} &  &  &  &  &  \\
\textbf{InternVL2\_5-8B-MPO correct} &  & 95.79 & 95.34 & 93.26 & 90.43 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  & 96.83 & 96.88 & 94.79 & 90.63 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  & 96.78 & 96.98 & 94.94 & 90.28 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on M3CoT (random)}
\label{tab:InternVL2_5-8B_M3CoT_TRAIN_random}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 62.42 & 59.92 & 59.75 & 58.46 & 57.42 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 62.42 & 59.36 & 58.93 & 58.63 & 58.54 \\
\textbf{InternVL2\_5-8B-MPO} &  & 68.98 & 67.64 & 66.22 & 61.56 \\
\textbf{InternVL2\_5-8B-MPO correct} &  & 69.15 & 67.69 & 65.96 & 63.46 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  & 68.94 & 68.12 & 67.00 & 64.32 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  & 69.72 & 68.59 & 65.88 & 63.72 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[!h]
\caption{InternVL2\_5-8B vs. InternVL2\_5-8B-MPO on M3CoT (jices)}
\label{tab:InternVL2_5-8B_M3CoT_TRAIN_jices}
\begin{tabular}{lccccc}
\toprule
 & 0-shot & 1-shot & 2-shot & 4-shot & 8-shot \\
\midrule
\textbf{InternVL2\_5-8B} & 62.42 & 60.83 & 60.18 & 60.87 & 60.01 \\
\textbf{InternVL2\_5-8B gt\_rationale} & 62.42 & 59.75 & 57.85 & 58.15 & 58.76 \\
\textbf{InternVL2\_5-8B-MPO} &  & 66.18 & 64.02 & 64.02 &  \\
\textbf{InternVL2\_5-8B-MPO correct} &  & 66.82 & 64.97 & 64.24 & 60.53 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale} &  & 68.81 & 68.59 & 67.56 & 64.62 \\
\textbf{InternVL2\_5-8B-MPO gt\_rationale correct} &  & 69.59 & 68.98 & 66.95 & 64.84 \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/models.tex <==
% \begin{table}[!h]
% \centering
% \begin{tabular}{c|c|c}
% \toprule
% \textbf{Base Model} & \textbf{Size} & \textbf{Reasoning Model} \\
% \midrule

% \multirow{6}{*}{Qwen2.5-VL}
%  & 3B  & VLM-R1 \\ \cmidrule{2-3}
%  & \multirow{3}{*}{7B}
%       & VL-Rethinker 7B \\
%  &   & R1-OneVision 7B \\
%  &   & OpenVL Thinker 7B \\ \cmidrule{2-3}
%  & \multirow{2}{*}{72B}
%       & VL-Rethinker 72B \\
%  &   & QVQ-72B-Preview \\

% \midrule

% \multirow{5}{*}{InternVL2.5}
%  & 4B  & InternVL2.5-4B-MPO \\ \cmidrule{2-3}
%  & \multirow{2}{*}{8B}  & InternVL2.5-8B-MPO \\
%  &     & MM-Eureka \\ \cmidrule{2-3}
%  & \multirow{2}{*}{38B}  & InternVL2.5-38B-MPO \\
%  &     & MM-Eureka-Zero \\ \cmidrule{2-3}
%  & 78B & InternVL2.5-78B-MPO \\

% \midrule

% Kimi-VL-A3B-Instruct & 3B  & Kimi-VL-A3B-Thinking \\

% \midrule

% Llama-3.2V           & 11B & LLaVA-CoT \\

% \bottomrule
% \end{tabular}
% \caption{Comparison of base models, sizes, and associated reasoning models.}
% \label{tab:reasoning_models}
% \end{table}




